MPI Progress For All

The progression of communication in the Message Passing Interface (MPI) is not well defined, yet it is critical for application performance, particularly in achieving effective computation and communication overlap. The opaque nature of MPI progress poses significant challenges in advancing MPI within modern high-performance computing (HPC) practices. Firstly, the lack of clarity hinders the development of explicit guidelines for enhancing computation and communication overlap in applications. Secondly, it prevents MPI from seamlessly integrating with contemporary programming paradigms, such as task-based runtimes and event-driven programming. Thirdly, it limits the extension of MPI functionalities from the user space. In this paper, we examine the role of MPI progress by analyzing the implementation details of MPI messaging. We then generalize the asynchronous communication pattern and identify key factors influencing application performance. Based on this analysis, we propose a set of MPI extensions designed to enable users to explicitly construct and manage an efficient progress engine. We provide example codes to demonstrate the use of these proposed APIs in achieving improved performance, adapting MPI to task-based or event-driven programming styles, and constructing collective algorithms that rival the performance of native implementations. Our approach is compared to previous efforts in the field, highlighting its reduced complexity and increased effectiveness.

==> discussion.tex <==
\section{Results}
To demonstrate the usage of our extensions, we implemented a user-level \texttt{MPI\_Allreduce} based on the recursive doubling algorithm~\cite{ruefenacht2017generalisation} and measured its performance against MPICH's internal implementation that uses the same algorithm. The result in Figure~\ref{fig:allreduce} shows that the custom user-level implementation  outperforms MPICH's native \texttt{MPI\_Iallreduce}. We believe this is due to the specific assumptions and shortcuts in the custom implementation. For example, we assume the number of processes is a power of 2 and that \texttt{sendbuf} is \texttt{MPI\_INPLACE}, which avoids certain checks and branches. Additionally, restricting to \texttt{MPI\_INT} and \texttt{MPI\_SUM} avoids a datatype switch and the function-call overhead of calling an operation function.
This highlights an advantage of custom code over an optimized MPI implementation: the former can leverage specific contexts from the application to avoid complexities and achieve greater efficiency.

\begin{figure}[t]
        \centering
        \includegraphics[width=0.6\textwidth]{images/allreduce.png}
        \caption{Custom single-integer allreduce latency vs \texttt{MPI\_Iallreduce}. Intel Xeon CPU E5-2695 v4 @ 2.10GHz, Omni-Path interconnect, one process per node.}
        \label{fig:allreduce}
\end{figure}


\section{Related Work}
Several related works address issues with MPI progress and the management of asynchronous tasks within MPI.

With MPICH and its derived MPI implementations, users can enable a dedicated background progress thread by setting a control variable. This is the simplest method for ensuring that MPI will always progress and complete any nonblocking operations, without requiring additional MPI calls from the application. However, this method has significant performance issues, including lock contention to the main thread and core oversubscription when process-per-node (PPN) is high. Thus, implicit async progress threads are generally not recommended.
MVAPICH~\cite{ruhela2019efficient} has proposed a design to address these issues by identifying scenarios where asynchronous progress is required and putting the async thread to sleep when it is not needed or beneficial. Their benchmarks showed up to a 60\% performance improvement over the original MPICH design. With the extension \texttt{MPIX\_Stream\_progress}, applications can easily implement the async progress thread within the application layer. The same tuning design as adopted in MVAPICH can be applied. Instead of the implementation detecting where async progress is required, the application can know where it is needed by design, thus controlling the progress thread more precisely and directly. \texttt{MPIX\_Stream\_progress} also allows applications to use MPIX streams to target async progress for specific contexts, thereby avoiding lock contention issues altogether. In contrast, it is difficult for an MPI implementation to detect user contexts or determine the scope of global progress.

Casper~\cite{casper} is a process-based asynchronous progress approach for MPI one-sided communication. It leverages one or more auxiliary ``ghost'' processes to offload communication progress for all application processes on a node. This approach addresses the thread contention and oversubscription issues of using progress threads and shows good benefits for passive-target RMA applications. Still, progress for passive-target RMA is not always straightforward using standard MPI APIs, which ultimately adds complexity to the Casper implementation. \texttt{MPIX\_Stream\_progress} can enable progress explicitly on specific resources, such as RMA windows, thereby keeping the code simpler and potentially more efficient by avoiding unnecessary global progress.

MPI includes an API called generalized requests, which allows users to wrap an asynchronous task into an MPI request, enabling it to be managed similarly to an MPI nonblocking operation.
While the generalized request behaves like a real MPI request (i.e., it can be passed to \texttt{MPI\_Test} or \texttt{MPI\_Wait}) it does not fulfill the primary purpose of users calling \texttt{MPI\_Test} or \texttt{MPI\_Wait}, which is to invoke progress on the nonblocking operation behind the request.
% There is no built-in progress mechanism for generalized requests; users are expected to progress the async task behind the generalized request outside of MPI.
% This raises questions about the usefulness of generalized requests. Since users don't rely on MPI to progress the task or query its status, a generalized MPI request is merely a redundant handle.
Indeed, a large-scale survey of MPI applications \cite{laguna2019large} found no usages of generalized requests. The few works in the literature that use generalized requests are all for implementing MPI APIs~\cite{hatanaka2017offloaded,latham2007extending} on top of a core implementation, necessitating the use of MPI requests. Interestingly, both works highlighted the lack of progress semantics in generalized requests and proposed adding a progress-polling callback to the interface.
The MPIX async extension proposed in this paper enables users to inject progress hooks into the MPI progress; thus, it perfectly complements the generalized request by providing a progression mechanism.

MPIX Schedule~\cite{schafer2019user} is a proposal to expose MPI's internal nonblocking collective system to applications so that users can create their own nonblocking collective algorithms or a series of coordinated MPI operations similar to a nonblocking MPI collective.
However, it is challenging for the MPIX Schedule to accommodate non-MPI operations. The proposal only has APIs to add operations represented as an MPI request or an MPI op. While it is possible to wrap a custom asynchronous operation via a generalized request, the usage is cumbersome. More critically, the lack of a progress mechanism limits the performance users can achieve compared to what is possible within an MPI implementation.
In contrast, the MPIX Async APIs address the root issue of providing interoperable MPI progress. Its simple yet flexible progress hook-based interface can accommodate arbitrary asynchronous tasks. Combined with generalized requests, it enables users to effectively experiment with MPI extensions, such as experimental collective algorithms, entirely from the application layer.

MPIX Continue~\cite{schuchart2021callback} is a proposal that allows MPI to call back a user-defined function upon the completion of a request, eliminating the need for the application to continuously test the request for completion.
The motivation behind the MPIX Continue APIs is to simplify the management of MPI requests within a task-based programming model. Task-based programming models often have their own task tracking, scheduling, and progression mechanisms. However, MPI's nonblocking interface requires applications to actively test or wait on individual requests, which can lead to thread contention and wasted CPU cycles due to redundant progression.
Our proposed extensions address directly many of the challenges that the MPIX Continue proposal seeks to resolve.
\texttt{MPIX\_Stream\_progress} can be used to implement a polling service that integrates with the task runtime system without requiring synchronization of MPI requests.
Meanwhile, \texttt{MPIX\_Request\_is\_complete} allows tasks to query the status of their dependent requests without triggering redundant progress invocations.
The \texttt{MPIX\_Async\_start} provides a progress callback interface that lets applications skip request tracking altogether. 

\section{Conclusions}
In summary, our proposal directly tackles the challenge of MPI progress by exposing it through explicit and extensible interfaces.
Our proposal empowers applications to directly manage MPI progress, allowing for fine-tuning of performance. By providing explicit control, applications can optimize communication patterns based on their specific requirements.
Beyond addressing immediate performance concerns, our proposal serves as a gateway for the HPC community to explore and enhance MPI beyond the confines of core implementations. It encourages experimentation, innovation, and the evolution of MPI in response to changing computing landscapes.


==> temp.tex <==
Strictly speaking, an MPI operation has parts: the initiation, the progress, and the synchronization.

Blocking operations have both the progress and synchronization bundled with the operations.

A nonblocking operation splits the operation between initiation and synchronization. However, how the progress taking place is somewhat undefined.

Use MPI\_Isend as an example, an implementation can complete the operation -- transfer the data to the NIC -- before the initiation call MPI\_Isend returns. This is typical when the message is small. In this case, the synchronization call such as MPI\_Wait will immediately return successful.
It is also possible that the initiation call merely pass the host memory address to the NIC and returns before the NIC finishes sending the entire message. If MPI\_Wait is called before the NIC finishes the transmission, MPI\_Wait will block until the transimission completes.
Lastly, MPI\_Isend may only initiate a handshake message to the receiver and will only start sending data when it receives the reply from receiver. In this case, without triggering progress, there is no actual progress in sending the data.

This asynchronous pattern can be generalized beyond network communication. IO. Collectives. GPU.

The asynchronous pattern is also popular in task-based programming paradigm.
Task-based programming allows programmers to decouple 
